Equilibria for Games with Combined Qualitative and Quantitative Objectives

The overall aim of our research is to develop techniques to reason about the equilibrium properties of multi-agent systems. We model multi-agent systems as concurrent games, in which each player is a process that is assumed to act independently and strategically in pursuit of personal preferences. In this article, we study these games in the context of finite-memory strategies, and we assume players' preferences are defined by a qualitative and a quantitative objective, which are related by a lexicographic order: a player first prefers to satisfy its qualitative objective (given as a formula of Linear Temporal Logic) and then prefers to minimise costs (given by a mean-payoff function). Our main result is that deciding the existence of a strict epsilon Nash equilibrium in such games is 2ExpTime-complete (and hence decidable), even if players' deviations are implemented as infinite-memory strategies.

==> notes.tex <==
\section{Notes}

Here are some other basic facts about $\LEX(\LTL,\mp)$-games that we should include.

\begin{enumerate}
 \item NE need not exist (matching pennies).
 \item Even if NE exist, they need not be positional. This is already true for mean-payoff games, cf.~\cite{DBLP:journals/corr/abs-1210-3539}.
 \item Mixed NE need not exist. Moreover, it is undecidable if there exists a mixed NE (already holds for mean-payoff).
\end{enumerate}

- positional strategies are strategies in which the suggested action only depends on the current state, not on the history

- finite-state strategies are strategies that can be implemented by finite-state transducers.


\subsection{Push weights into the states}
	This is done by replacing $St$ by $St \times Act^{Ag}$ and defining the weight of $(s,d)$ to be $\kappa(d)$.
	Formally, we obtain a state-weighted arena $A' = (AG, Act, Ap, W, St', \iota', tr', \lambda, (\kappa'_{a})_{a \in Ag})$ with $\kappa'_a: St' \to W$, such that
	
	\begin{itemize}
		\item
			$St' = St \times Act^{Ag}$;
			
		\item
			$\iota' = (\iota, d)$ for some $d \in Act^{Ag}$;
			
		\item
			$\lambda'(s,d) = \lambda(s)$;
			
		\item
			$\kappa'_a(s,d) = \kappa_a(d_a)$;
			
		\item
			$tr'((s,d), d') = (tr(s,d'), d')$.
	\end{itemize}
	
	
	Games on state-weighted arenas are defined as before: simply note that one can extend $\kappa'_a$ to executions, 
	i.e., for $\pi = t_0 d_0 t_1 d_1 \dots$, define $\kappa'_a(\pi) = \kappa_a(t_0) \kappa_a(t_1) \cdots$.
	
	\begin{lemma}
		\label{lmm:ltltoparity}
		For every $\epsilon > 0$ and every \LEX(\buchi, \mp) game $G = (A, \Psi)$, it holds that $\NE^\epsilon(G) = \NE^\epsilon(A',\Psi)$.
	\end{lemma}
	
	\begin{proof}
%		
		\todo{missing}
%		
%		By construction we have that $\NE(G) = \NE(G)$.
%	
%		Observe that $A$ and $A'$ have the same set of agents and action. Thus, due to Remark~\ref{rmk:actstrat} we can assume they have the same set of strategies.
%		It is not hard to see that a strategy profile is a Nash Equilibrium in  $G= (A, \Psi)$ if and only if it is so in $G = (A', \Psi)$ too.
	\end{proof}
	
	Thus, without loss of generality, we assume that $G$ has weights on the states.
\subsection{text about reduction}
The idea is that a finite-state $\epsilon$
Nash-equilibrium induces an ultimately periodic path in a certain subgraph of
the arena such that the payoff of this path is at least a certain threshold.
This approach is inspired by the proof that one can decide the existence of (not
neccessarily finite-state) Nash equilibria in mean-payoff
games~\cite{DBLP:conf/concur/UmmelsW11}. However, in order to deal with the more
complicated objectives (i.e., $\LEX(\buchi,\mp)$ instead of simply mean-payoff),
and in order to deal with the fact that we are restricting to finite-state
profiles, we need additional ideas. In particular, we supply a careful study of
two-player zero-sum games $H$ with $\LEX(\buchi,\mp)$ objectives, and show that
i) these games have values $v(G)$, and ii) for every $\epsilon$ there is a
finite-state strategy for the minimiser that achieves at most $v(G) + \epsilon$.
The proof of this fact is inspired by similar reasonings for energy-parity games
and mean-payoff parity games~\cite{}.

\subsection{Text for Buchi mean-payoff games}
The minimiser can play optimally using
infinite-state strategies that alternate between two phases: at even phases it
uses a memoryless strategy to force a visit to a B\"uchi state, and in odd
phases it applies a memoryless strategy that maximises the mean-payoff. There is
a bound on the number of time steps each even phase takes, while infinite-memory
is used to play the odd-phases for longer and longer time steps. We then show
that, given $\epsilon > 0$ there is a bound $B$ such that the finite-state
strategy that behaves similarly except that it caps the time in each odd-phase
to $B$ time steps, achieves a value at most $\epsilon$ more than the optimal
value.


